HM3D-ABO: A Photo-realistic Dataset for Object-centric Multi-view 3D Reconstruction

Reconstructing 3D objects is an important computer vision task that has wide application in AR/VR. Deep learning algorithm developed for this task usually relies on an unrealistic synthetic dataset, such as ShapeNet and Things3D. On the other hand, existing real-captured object-centric datasets usually do not have enough annotation to enable supervised training or reliable evaluation. In this technical report, we present a photo-realistic object-centric dataset HM3D-ABO. It is constructed by composing realistic indoor scene and realistic object. For each configuration, we provide multi-view RGB observations, a water-tight mesh model for the object, ground truth depth map and object mask. The proposed dataset could also be useful for tasks such as camera pose estimation and novel-view synthesis. The dataset generation code is released at https://github.com/zhenpeiyang/HM3D-ABO.

==> shape_qualitative.tex <==

\begingroup
\setlength{\tabcolsep}{1.0pt} % Default value: 6pt
% \renewcommand{\arraystretch}{0.8} % Default value: 1
   \begin{figure*}[!ht]
    %  \centering
    \hspace{-1em}
     \def\imw{0.14\textwidth}
     \def\imh{0.08\textheight}

     \begin{tabular}{ccccccc}

        
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/n2Tt2eJdqnT_B07M7NRPZR_016_040_019_064/000016.jpg} & 
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/n2Tt2eJdqnT_B07M7NRPZR_016_040_019_064/000019.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/n2Tt2eJdqnT_B07M7NRPZR_016_040_019_064/000040.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/n2Tt2eJdqnT_B07M7NRPZR_016_040_019_064/000064.jpg} &
      \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/idr_n2Tt2eJdqnT_B07M7NRPZR_016_040_019_064_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/onet_n2Tt2eJdqnT_B07M7NRPZR_016_040_019_064_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/ours_n2Tt2eJdqnT_B07M7NRPZR_016_040_019_064_crop.png} \\

     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/tj8ngv3woJ3_B07HSKB7B4_037_024_059_023/000023.jpg} & 
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/tj8ngv3woJ3_B07HSKB7B4_037_024_059_023/000024.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/tj8ngv3woJ3_B07HSKB7B4_037_024_059_023/000037.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/tj8ngv3woJ3_B07HSKB7B4_037_024_059_023/000059.jpg} &
      \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/idr_tj8ngv3woJ3_B07HSKB7B4_037_024_059_023_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/onet_tj8ngv3woJ3_B07HSKB7B4_037_024_059_023_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/ours_tj8ngv3woJ3_B07HSKB7B4_037_024_059_023_crop.png} \\

     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/udze1CSof5C_B0735WMNT5_012_024_031_035/000012.jpg} & 
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/udze1CSof5C_B0735WMNT5_012_024_031_035/000024.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/udze1CSof5C_B0735WMNT5_012_024_031_035/000031.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/udze1CSof5C_B0735WMNT5_012_024_031_035/000035.jpg} &
      \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/idr_udze1CSof5C_B0735WMNT5_012_024_031_035_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/onet_udze1CSof5C_B0735WMNT5_012_024_031_035_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/ours_udze1CSof5C_B0735WMNT5_012_024_031_035_crop.png} \\
        
        
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/1Rg1SS1dRpG_B07TN2RRDG_037_022_035_042/000022.jpg} & 
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/1Rg1SS1dRpG_B07TN2RRDG_037_022_035_042/000035.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/1Rg1SS1dRpG_B07TN2RRDG_037_022_035_042/000037.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/1Rg1SS1dRpG_B07TN2RRDG_037_022_035_042/000042.jpg} &
      \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/idr_1Rg1SS1dRpG_B07TN2RRDG_037_022_035_042_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/onet_1Rg1SS1dRpG_B07TN2RRDG_037_022_035_042_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/ours_1Rg1SS1dRpG_B07TN2RRDG_037_022_035_042_crop.png} \\
        
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/bwoBmU23M2N_B07QGWN1Y1_005_024_031_002/000002.jpg} & 
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/bwoBmU23M2N_B07QGWN1Y1_005_024_031_002/000005.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/bwoBmU23M2N_B07QGWN1Y1_005_024_031_002/000024.jpg} &
     \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/bwoBmU23M2N_B07QGWN1Y1_005_024_031_002/000031.jpg} &
      \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/idr_bwoBmU23M2N_B07QGWN1Y1_005_024_031_002_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/onet_bwoBmU23M2N_B07QGWN1Y1_005_024_031_002_crop.png}&
        \includegraphics[height=\imh, width=\imw, keepaspectratio]{Figures/habitat_results/ours_bwoBmU23M2N_B07QGWN1Y1_005_024_031_002_crop.png} \\
        
        
             \multicolumn{4}{c}{Few-view Input} & IDR~\cite{idr} & OccNet$^\dagger$~\cite{mescheder2019occupancy,apple} &FvOR~\cite{yang2022fvor}
	 \end{tabular}
     \vspace{-5pt}
     \caption{Qualitative comparisons between three approaches on HM3D-ABO. For each column, we show the 4 input views on the left and the reconstruction of each method on the right. FvOR~\cite{yang2022fvor} and IDR~\cite{idr} use pose predicted by FvOR-Pose~\cite{yang2022fvor}.}
     \label{fig:visualization}\vspace{-1mm}
   \end{figure*}
\endgroup


==> symbols.tex <==
\let \bs = \boldsymbol
%\newcommand{\classset}{\mathcal{C}}
\let \set = \mathcal

\newcommand{\pos}{\mathbf{p}}
\newcommand{\vertex}{\bs{v}}
\newcommand{\edge}{\bs{e}}
\newcommand{\pred}{0}
\newcommand{\init}{\textup{init}}
\newcommand{\pose}{\textup{pose}}
\newcommand{\GMM}{M}
\newcommand{\GAMMA}{\Gamma}
\newcommand{\graph}{\mathcal{G}}
\newcommand{\vertexset}{\mathcal{V}}
\newcommand{\edgeset}{\mathcal{E}}
\newcommand{\edgeweightset}{\mathcal{W}}
\newcommand{\edgeweight}{w}
\newcommand{\normalizededgeweight}{\hat{w}}

\newcommand{\gt}{\textup{gt}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\klloss}{\loss_{KL}}

\newcommand{\argmin}{\arg\min}

\newcommand{\ps}{\mathcal{P}}

\DeclareMathOperator{\Tr}{Tr}

\newcommand{\smooth}{\textup{smooth}}
\newcommand{\p}{\bs{p}}
\newcommand{\q}{\bs{q}}
\newcommand{\ro}{\bs{r}} 
\newcommand{\tn}{\bs{t}} % translation
\newcommand{\n}{\bs{n}} % normal
\newcommand{\om}{\bs{\omega}} % Lie algebra

\newcommand{\vf}{\bs{v}} % vertex feature
\newcommand{\ef}{\bs{e}} % edge feature

\newcommand{\T}{\bs{T}} % Transformation

\newcommand{\R}{\mathcal{R}}
\newcommand{\Q}{\bs{Q}}
\newcommand{\W}{\bs{W}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\skewm}[1]{\left[#1\right]_{\times}}

\newcommand{\primitive}{p}

